CAM-Convs: Camera-Aware Multi-Scale Convolutions for Single-View Depth

Single-view depth estimation suffers from the problem that a network trained on images from one camera does not generalize to images taken with a different camera model. Thus, changing the camera model requires collecting an entirely new training dataset. In this work, we propose a new type of convolution that can take the camera parameters into account, thus allowing neural networks to learn calibration-aware patterns. Experiments confirm that this improves the generalization capabilities of depth prediction networks considerably, and clearly outperforms the state of the art when the train and test images are acquired with different cameras.

==> paper/sections/old_experiments_focal_sensor.tex <==
\subsection{Training and testing with multiple focal lengths}

In this experiment we evaluate the performance of a standard U-Net architecture, with and without focal length normalization, when it is trained and tested on images with different camera parameters.

%

The results can be found in Table \ref{tab:focal_norm_simple}. We generated $3$ test sets, each one with a different focal length, and $6$ training sets for each test set. The training sets were generated with one focal length, two focal lengths (with the same probability), or random ones distributed in an interval. We will take as baselines the networks trained and tested in images with the same focal length, without focal length normalization (in orange) and with it (in blue).

Several things should be noticed here. First, the overfit: Even with focal normalization, the performance of a network degrades when tested on focal lengths different from the training ones. See, for example, the error metrics of the $1^{st}$ row (training and test images with focal length \extraFocalR{}) and their degradation in the $2^{nd}$ and $3^{rd}$ rows (test images with focal length \extraFocalR{} and training ones with focal lengths \smallFocalR{} and \bigFocalR{} respectively). Focal normalization, then, has limitations to generalize to unseen cameras.

The results improve when the training set contains images with different focal lengths. See, for example, for the test set \extraFocalR{}, that the network trained on focal lengths \smallFocalR{}\bigFocalR{} is closer to the baseline (in orange).

%


%

Notice, finally, that normalizing the focal length improves significantly the performance when training on data with different focal lengths. Compare, for example, the error metrics of the rows \smallFocalR{}\bigFocalR{}$^*$ and \smallFocalR{}\bigFocalR{}. Notice that changes in the focal length can produce inconsistencies on the data, as they produce changes on the image size of the objects that do not depend on the depth. Networks trained on \smallFocalR{}\bigFocalR{}$^*$, in fact, did not converge easily. Focal length normalization alleviates such inconsistencies. 

However, focal length normalization has two limitations: First, it does not model the changes on the sensor size and the resolution (that we will address in the next subsection). And second, Equation \ref{eq:normalizeddepth} only holds if the pixel size is the same for every camera in the training and test sets, which in general is not the case.

%

%


\subsection{Training and testing with multiple sensor sizes}

%

Although Fully Convolutional Networks (FCN) can be applied to any sensor size, they do not generalize well due to context dependency. In this experiment we evaluate different networks trained on 3 sizes (\bigImR{}, \bigImtR{} and \sqImR{}). In order to reduce the influence of context, we train and test on random focal lengths ($\mathcal{U}$\smallFocalR{}\bigFocalR{}) using focal normalization. We train on the different sizes separately and combining different sizes. We train with multiple sizes by training two networks with weight sharing (Siamese Networks). The results of this experiment are shown in Table \ref{tab:diffimsizemean_simple}. We can observe several things.

Networks {\color{baseline2} trained on a sensor size and tested on other} do not perform as well as ({\color{baseline1} networks trained and tested on the same sensor size}. Single-view depth estimation is a context dependent task, and the network overfits to the amount of context in the training sensor size. Training with multiple sensor sizes does not make the network perform better than the baselines but reduces the error. %
Further, training a stack of weight sharing networks also does not scale to large numbers of different sensor sizes.

    %
    %





\input{paper/tables/sensor_size_resize_kitti_scannet.tex}

We perform a similar experiment with two public datasets: KITTI \cite{Uhrig2017THREEDV}, with sensor size \kittiSizeR{}$=384\times128$; and ScanNet \cite{dai2017scannet}, with sensor size \scannetSizeR{}$=256\times192$. The change is larger than the previous experiment. Results are reported on Table \ref{tab:diffsizekittiscan}. Notice that, in this case, training with both sensor sizes decreased the performance. However, for our surprise, a simple resizing policy proved to work as good as the baselines, models trained only on one dataset ({\color{baseline1} orange} lines in the table). Notice that this resize option will deform images aspect ratio. It also implies the recalculation of a new average focal length $f_r=f\frac{r_x+r_y}{2}$ for normalization \todo{ben: is the kitti and scannet experiment with normalization?} (where $r_x$ and $r_y$ are the resizing factors for the horizontal and vertical dimensions of the image).

%
%
%

%


%

Resizing worked in this case because of the completely different distribution of the two datasets, with null intersection of features (\textit{e.g.} there are no chairs on KITTI and no cars on ScanNet). Resizing did not create inconsistent data during training. In order to prove this point, we tested the resizing on the 2D-3D Stanford dataset. See the results in Table \ref{tab:resizing}. In this case, the performance degradation introduced by resizing is noticeable.

%

%

As a summary, FCN networks cannot generalize to sensor sizes different from the training ones. Training with different sensor sizes, the test one included, cannot improve the results over training with the test sensor size. This suggests that the network is not exploiting the extra data. Image resizing helps in the case of completely different data distributions, but degrades the performance otherwise. In the next subsection we show how \shortConvs{} are able to generalize in all the cases, outperforming the baselines when training on different sensor sizes.

%


==> paper/tables/first_table_camconvs.tex <==
\begin{table}
\centering
\begin{threeparttable}[b]
\begin{tabular}{=c+c+c+c+c+c+c+c+c+c}
%
%
\textbf{Test} & \textbf{Train}& abs.rel&l1.inv&rmse&sc.inv  \\
\hline
 &  & $:1$ & $1/m$ & $1/m$ & $lg(m)$ \\

\multirow{ 2}{*}{\bigImR{}} 
\rowstyle{\color{baseline1}}
  &\multirow{ 1}{*}{\bigImR{}}
  	&$0.189$ &$0.15$ &$0.46$ &$0.037$\\%200000
  &\multirow{ 1}{*}{\withBoxNet{}\tnote{\ddag}}  
    &$\mathbf{0.175}$ &$\mathbf{0.144}$ &$\mathbf{0.433}$ &$\mathbf{0.0312}$ \\ 
    
  \hline
  
  
 \multirow{ 2}{*}{\bigImtR{}}  
    \rowstyle{\color{baseline1}}
  &\multirow{ 1}{*}{\bigImtR{}}
&$0.166$ &$0.133$ &$0.412$ &$0.0323$\\%200000
&\multirow{ 1}{*}{\withBoxNet{}\tnote{\ddag}} 
    &$\mathbf{0.158}$ &$\mathbf{0.131}$ &$\mathbf{0.39}$ &$\mathbf{0.0265}$\\
    
  \hline
  
  \rowstyle{\color{baseline1}}
  \multirow{ 2}{*}{\sqImR{}} 
  &\multirow{ 1}{*}{\sqImR{}}
  	&$0.174$ &$0.14$ &$0.425$ &$0.0336$\\%200000
    &\multirow{ 1}{*}{\withBoxNet{}\tnote{\ddag}} 
    &$\mathbf{0.164}$ &$\mathbf{0.134}$ &$\mathbf{0.402}$ &$\mathbf{0.0283}$\\
  	\cline{3-7}
  \multicolumn{2}{c}{}&\multicolumn{4}{c}{\stb{}}
  
\end{tabular}
\begin{tablenotes}
    %
    \item[\ddag] Trained with weight sharing in sensor sizes \bigImR{} and \bigImtR{}.
\end{tablenotes}
\end{threeparttable}
\\
\caption{\label{tab:camconvs1_simple} Results on training and testing on multiple sensor sizes. $1^{st}$ column: sensor size for test set. $2^{nd}$ column: sensor size or sizes during training. This is a continuation of Table \ref{tab:diffimsizemean_simple}. All the models were trained and tested with uniformly sampled focal length between $\smallFocal{}$ and $\bigFocal{}$.}
\end{table}

==> paper/tables/focal_length.tex <==
\begin{table}[t!]
\centering
\begin{threeparttable}[b]
\begin{tabular}{@{\extracolsep{4pt}}=c+c+c+c+c}
\textbf{Test f} & \textbf{Train f}&l1.inv&rmse&sc.inv\\
\hline
$pixels$ & $pixels$ & $1/m$ & $m$ & $lg(m)$\\
\rowstyle{\color{baseline1}}
\multirow{ 7}{*}{\extraFocalR{}} 
  &\multirow{ 1}{*}{\extraFocalR{}\tnote{*}}
  	   &$\mathbf{0.184}$ &$\mathbf{0.378}$ &$\mathbf{0.0347}$ \\%200000
  &\multirow{ 1}{*}{\smallFocalR{}}
  	  &$0.193$ &$0.395$ &$\mathbf{0.0354}$\\%200000
  &\multirow{ 1}{*}{\bigFocalR{}}
  	 &$0.318$ &$0.572$ &$0.0483$ \\%200000
   &\multirow{ 1}{*}{\footnotesize\smallFocalR{}\bigFocalR{}\tnote{*}}
  	 &$0.659$ &$0.864$ &$0.0614$ \\%200000
   &\multirow{ 1}{*}{\footnotesize\smallFocalR{}\bigFocalR{}}
  	 &$\mathbf{0.189}$ &$\mathbf{0.387}$ &$0.0361$\\%200000
   &\multirow{ 1}{*}{\footnotesize$\mathcal{U}$\smallFocalR{}\bigFocalR{}}
  	 &$0.194$ &$0.398$ &$0.0374$ \\%200000
\hline
\rowstyle{\color{baseline1}}
\multirow{ 6}{*}{\smallFocalR{}} 
  &\multirow{ 1}{*}{\smallFocalR{}\tnote{*}}
  	&$\mathbf{0.17}$ &$\mathbf{0.4}$ &$\mathbf{0.0354}$ \\%200000
\rowstyle{\color{baseline2}}  &\multirow{ 1}{*}{\smallFocalR{}}
  	 &$0.174$ &$0.407$ &$0.0364$\\%200000
  &\multirow{ 1}{*}{\bigFocalR{}}
  	 &$0.272$ &$0.564$ &$0.0459$ \\%200000
   &\multirow{ 1}{*}{\footnotesize\smallFocalR{}\bigFocalR{}\tnote{*}}
  	&$0.552$ &$0.888$ &$0.0609$\\%200000
   &\multirow{ 1}{*}{\footnotesize\smallFocalR{}\bigFocalR{}}
  	 &$\mathbf{0.175}$ &$\mathbf{0.404}$ &$\mathbf{0.0364}$ \\%200000
   &\multirow{ 1}{*}{\footnotesize$\mathcal{U}$\smallFocalR{}\bigFocalR{}}
  	 &$0.179$ &$0.414$ &$0.0378$ \\%200000

\hline
\rowstyle{\color{baseline1}}
\multirow{ 6}{*}{\bigFocalR{}} 
  &\multirow{ 1}{*}{\bigFocalR{}\tnote{*}}
  	 &$0.141$ &$0.51$ &$0.0387$ \\%200000
  &\multirow{ 1}{*}{\smallFocalR{}}
  	 &$0.133$ &$0.524$ &$0.0411$ \\%200000
\rowstyle{\color{baseline2}}  &\multirow{ 1}{*}{\bigFocalR{}}
  	 &$0.149$ &$0.532$ &$0.0396$ \\%200000
   &\multirow{ 1}{*}{\footnotesize\smallFocalR{}\bigFocalR{}\tnote{*}}
  	 &$0.208$ &$0.813$ &$0.063$ \\%200000
&\multicolumn{3}{c}{\todo{ben: are the numbers in the row above correct?}}\\ %
&\multicolumn{3}{c}{\todo{jm: they were not, now they are}}\\ %
   &\multirow{ 1}{*}{\footnotesize\smallFocalR{}\bigFocalR{}}
  	 &$\mathbf{0.132}$ &$\mathbf{0.504}$ &$\mathbf{0.038}$ \\%200000
   &\multirow{ 1}{*}{\footnotesize$\mathcal{U}$\smallFocalR{}\bigFocalR{}}
  	 &$0.134$ &$0.512$ &$0.0385$ \\%200000
\cline{3-5}
\multicolumn{2}{c}{}&\multicolumn{3}{c}{\stb{}}\\
\end{tabular}
\begin{tablenotes}
  \item[*] trained without focal length normalization.
\end{tablenotes}
\end{threeparttable}
\\
\caption{\label{tab:focal_norm_simple}Influence of focal length normalization.  We normalize our predictions focal length so that the network assumes \normFocalR{}$=\normFocal{}$.
$1^{st}$ column: Focal length of the test set. $2^{nd}$ column: Focal length of the training set. (\smallFocalR{}\bigFocalR{} means two focals at training, and $\mathcal{U}$\smallFocalR{}\bigFocalR{} stands for a uniform distribution between \smallFocalR{} and \bigFocalR{}). $3^{rd}$ to $5^{th}$ column: Error metrics. The baselines are: In {\color{baseline1} orange}, same focal length at train and test and no focal normalization. In {\color{baseline2} blue}, same focal length at train and test and focal normalization.}
\end{table}

==> paper/tables/second_table_camconvs.tex <==
\begin{table}
\centering
\begin{threeparttable}[b]
\begin{tabular}{=c+c+c+c+c+c+c+c+c}
%
%
 \textbf{Train}& abs.rel&l1.inv&rmse&sc.inv  \\
\hline
  & $:1$ & $1/m$ & $1/m$ & $lg(m)$ \\


\rowstyle{\color{baseline1}}
  \multirow{ 1}{*}{\centering\extraImR{}-\extraFocalR{}}
  	&$\mathbf{0.163}$ &$\mathbf{0.227}$ &$0.309$ &$\mathbf{0.0356}$\\%200000
  	
  \multirow{ 1}{*}{\centering\bigImR{}-\extraFocalR{}} 
  	&$0.245$ &$0.292$ &$0.337$ &$0.0598$\\	
  	
  \multirow{ 1}{*}{\footnotesize\centering\bigImR{}\bigImtR{}-$\mathcal{U}$\smallFocalR{}\bigFocalR{}}
    &$0.369$ &$0.369$ &$0.44$ &$0.0427$	\\
  	
  %
  %
    
  \multirow{ 1}{*}{\withBoxNet{}\tnote{\ddag}}  
    &$\mathbf{0.177}$ &$\mathbf{0.236}$ &$\mathbf{0.289}$ &$\mathbf{0.0362}$ \\ 
    
   %
  
  
  	\cline{2-6}
  \multicolumn{1}{c}{}&\multicolumn{4}{c}{\stb{}}
  
\end{tabular}
\begin{tablenotes}
    %
    \item[\ddag] trained with weight sharing in sensor sizes \bigImR{} and \bigImtR{}. Focal length is $\mathcal{U}$\smallFocalR{}\bigFocalR{}.
\end{tablenotes}
\end{threeparttable}
\\
\caption{\label{tab:camconvs2_simple} Results for test set with sensor size \extraImR{} and fixed focal length \extraFocalR{}. The baseline ($1^{st}$ row in {\color{baseline1}orange}) is a network trained on the exact same camera. The $2^{nd}$ network is trained with the same focal but different sensor size. The rest of the networks are trained with random focal lengths, uniformly distributed between $\smallFocal{}$ and $\bigFocal{}$. See how \shortConvs{} generalize to completely unseen camera models.}
\end{table}

==> paper/tables/sensor_size.tex <==
\begin{table}
\centering
\begin{threeparttable}[b]
\begin{tabular}{=c+c+c+c+c+c+c+c+c+c}
%
%
\textbf{Test} & \textbf{Train}& abs.rel&l1.inv&rmse&sc.inv  \\
\hline
 &  & $:1$ & $1/m$ & $m$ & $lg(m)$ \\

\multirow{ 5}{*}{\bigImR{}} 
\rowstyle{\color{baseline1}}
  &\multirow{ 1}{*}{\bigImR{}}
  	&$0.189$ &$\mathbf{0.15}$ &${\mathbf{0.46}}$ &${\mathbf{0.037}}$\\%200000
    \rowstyle{\color{baseline2}}
  &\multirow{ 1}{*}{\bigImtR{}}
&$0.206$ &$0.175$ &$0.51$ &$0.0422$\\%200000
\rowstyle{\color{baseline2}}
  &\multirow{ 1}{*}{\sqImR{}}
  	&$0.193$ &$0.158$ &$0.476$ &$0.0378$\\%200000
    %
  &\multirow{ 1}{*}{\centering\bigImR{} \bigImtR{}}
  	&$0.191$ &$0.153$ &$0.484$ &$0.0401$\\%200000
    
  %
    %
  &\multirow{ 1}{*}{\footnotesize\centering\bigImR{} \bigImtR{} \sqImR{}}
  	&${\mathbf{0.184}}$ &${0.154}$ &${0.464}$ &${0.0424}$\\%200000
  %
  %
  \hline
  
  
  \multirow{ 5}{*}{\bigImtR{}} 
\rowstyle{\color{baseline2}}
  &\multirow{ 1}{*}{\bigImR{}}
  	&$0.197$ &$0.151$ &$0.44$ &$0.038$ \\%200000
    \rowstyle{\color{baseline1}}
  &\multirow{ 1}{*}{\bigImtR{}}
&${\mathbf{0.166}}$ &${\mathbf{0.133}}$ &$\mathbf{0.412}$ &$\mathbf{0.0323}$\\%200000
\rowstyle{\color{baseline2}}
  &\multirow{ 1}{*}{\sqImR{}}
  		&$0.174$ &$0.138$ &$0.42$ &$0.0334$\\%200000
    %
  &\multirow{ 1}{*}{\centering\bigImR{} \bigImtR{}}
  	&$0.173$ &$0.139$ &$0.436$ &$0.0352$\\%200000
    
  %
    %
  &\multirow{ 1}{*}{\footnotesize\centering\bigImR{} \bigImtR{} \sqImR{}}
  	&${0.168}$ &${0.14}$ &${0.422}$ &$0.0376$\\%200000
  %
  %
  \hline
  
  
  \multirow{ 5}{*}{\sqImR{}} 
\rowstyle{\color{baseline2}}
  &\multirow{ 1}{*}{\bigImR{}}
  	&$0.184$ &$0.143$ &$0.44$ &$0.0357$\\%200000
    \rowstyle{\color{baseline2}}
  &\multirow{ 1}{*}{\bigImtR{}}
&$0.177$ &$0.145$ &$0.435$ &$0.0356$\\%200000
\rowstyle{\color{baseline1}}
  &\multirow{ 1}{*}{\sqImR{}}
  	&$0.174$ &$\mathbf{0.14}$ &${\mathbf{0.425}}$ &${\mathbf{0.0336}}$\\%200000
    %
  &\multirow{ 1}{*}{\centering\bigImR{} \bigImtR{}}
  	&$0.178$ &$0.143$ &$0.451$ &$0.0365$\\%200000
    
  %
   %
  &\multirow{ 1}{*}{\footnotesize\centering\bigImR{} \bigImtR{} \sqImR{}}
  &${\mathbf{0.171}}$ &${0.143}$ &${0.432}$ &${0.0383}$\\%200000
  %
 %
  	\cline{3-7}
  \multicolumn{2}{c}{}&\multicolumn{4}{c}{\stb{}}
  
\end{tabular}
%
    %
    %
%
\end{threeparttable}
\\
\caption{\label{tab:diffimsizemean_simple}Results for training and testing on different sensor sizes. $1^{st}$ column: Sensor size of test set. $2^{nd}$ column: Sensor size of training set. $3^{rd}$ to $6^{th}$ columns: Error metrics.}
\end{table}
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
    
%
%
%
%
%
%
%
%
%
%
  
  
%
%
%
%
%
%
%
%
%
%
%
%
%
    
%
%
%
%
%
%
%
%
%
%
  
  
%
%
%
%
%
%
%
%
%
%
%
%
%
    
%
%
%
%
%
%
%
%
%
%
%
  
%
%
%
%
%
%
%
%
%

==> paper/tables/sensor_size_resize.tex <==
\begin{table}
\centering
\begin{threeparttable}[b]
\begin{tabular}{=c+c+c+c+c+c+c+c+c+c}
%
%
\textbf{Test} & \textbf{Train}& abs.rel&l1.inv&rmse&sc.inv  \\
\hline
 &  & $:1$ & $1/m$ & $m$ & $lg(m)$ \\

\multirow{ 2}{*}{\bigImR{}} 
  
  &\multirow{ 1}{*}{\footnotesize\centering\bigImR{} \bigImtR{} \sqImR{}}
  	&${\mathbf{0.184}}$ &$\mathbf{0.154}$ &$\mathbf{0.464}$ &$\mathbf{0.0424}$\\%200000
  &\multirow{ 1}{*}{\footnotesize\centering\bigImR{} \bigImtR{}\tnote{\textdagger} \sqImR{}\tnote{\textdagger}}&$0.239$ &$0.179$ &$0.742$ &$0.064$\\%200000

  \hline
  
  
  \multirow{ 2}{*}{\bigImtR{}} 
  &\multirow{ 1}{*}{\footnotesize\centering\bigImR{} \bigImtR{} \sqImR{}}
  	&$\mathbf{0.168}$ &$\mathbf{0.14}$ &$\mathbf{0.422}$ &$\mathbf{0.0376}$\\%200000
  &\multirow{ 1}{*}{\footnotesize\centering\bigImR{} \bigImtR{}\tnote{\textdagger} \sqImR{}\tnote{\textdagger}}	&$0.209$ &$0.16$ &$0.622$ &$0.0514$\\%200000
 
  \hline
  
  
  \multirow{ 2}{*}{\sqImR{}} 

  &\multirow{ 1}{*}{\footnotesize\centering\bigImR{} \bigImtR{} \sqImR{}}
  &${\mathbf{0.171}}$ &$\mathbf{0.143}$ &$\mathbf{0.432}$ &$\mathbf{0.0383}$\\%200000
  &\multirow{ 1}{*}{\footnotesize\centering\bigImR{} \bigImtR{}\tnote{\textdagger} \sqImR{}\tnote{\textdagger}}  	&$0.219$ &$0.164$ &$0.662$ &$0.0552$\\%200000
  	\cline{3-7}
  \multicolumn{2}{c}{}&\multicolumn{4}{c}{\stb{}}
  
\end{tabular}
\begin{tablenotes}
    %
    \item[\textdagger] sensor size has been resized to the first one in the list.
\end{tablenotes}
\end{threeparttable}
\\
\caption{\label{tab:resizing}Results for training and testing on different sensor sizes. Notice that resizing does not generalize over multiple cameras.}
\end{table}
